Maximizing Determinants under Matroid Constraints

Given vectors $v_1,\dots,v_n\in\mathbb{R}^d$ and a matroid $M=([n],I)$, we study the problem of finding a basis $S$ of $M$ such that $\det(\sum_{i \in S}v_i v_i^\top)$ is maximized. This problem appears in a diverse set of areas such as experimental design, fair allocation of goods, network design, and machine learning. The current best results include an $e^{2k}$-estimation for any matroid of rank $k$ and a $(1+\epsilon)^d$-approximation for a uniform matroid of rank $k\ge d+\frac d\epsilon$, where the rank $k\ge d$ denotes the desired size of the optimal set. Our main result is a new approximation algorithm with an approximation guarantee that depends only on the dimension $d$ of the vectors and not on the size $k$ of the output set. In particular, we show an $(O(d))^{d}$-estimation and an $(O(d))^{d^3}$-approximation for any matroid, giving a significant improvement over prior work when $k\gg d$. Our result relies on the existence of an optimal solution to a convex programming relaxation for the problem which has sparse support; in particular, no more than $O(d^2)$ variables of the solution have fractional values. The sparsity results rely on the interplay between the first-order optimality conditions for the convex program and matroid theory. We believe that the techniques introduced to show sparsity of optimal solutions to convex programs will be of independent interest. We also give a randomized algorithm that rounds a sparse fractional solution to a feasible integral solution to the original problem. To show the approximation guarantee, we utilize recent works on strongly log-concave polynomials and show new relationships between different convex programs studied for the problem. Finally, we use the estimation algorithm and sparsity results to give an efficient deterministic approximation algorithm with an approximation guarantee that depends solely on the dimension $d$.

==> NSW.tex <==


In the indivisible goods allocation problem the goal is allocate, i.e., partition $m$ goods among $d$ agents, so that some notion of social welfare and/or fairness is achieved. Suppose that $S_i$ are the goods allocated to agent $i$. The agent then has utility $u_i(j)$ for every good $j \in [m]$, and it is common to assume that her utility $u_i(S_i)$ for the set of goods allocated to her is additive, i.e.~$u_i(S_i) = \sum_{j   \in S_i}{u_i(j)}$.  A well studied objective in this contest is Nash social welfare (NSW), which asks to maximize the geometric mean $\left(\prod_{i =     1}^du_i(S_i)\right)^{1/d}$ of the utilities of the layers. Intuitively, this objective favors allocations with more equal distribution of the utility, and provides a trade-off between the additive social welfare, which can lead to allocations that give all goods to a single agent, and the max-min social welfare, which can lead to inefficient allocations: see ~\cite{moulin,CKMPSW16} for more extensive background. Maximizing the NSW can be formulated as a determinant maximization problem over a partition constraint, as observed in~\cite{anari2016nash}. For each agent $i$ and good $j$, we create a vector $\bv_{(i,j)} = \sqrt{u_i(j)} \be_i$, where $\be_i$ is the $i$-th standard basis vector of $\R^d$. We also form a partition matroid $\M$, whose bases $\B$ consist of all sets $S \subseteq [d] \times [m]$ such that $|\{i: (i,j) \in S\}| = 1$ for all $j \in [m]$. Then, a feasible solution $S \in \B$ corresponds exactly to an allocation of the goods, and the determinant $\det\left(\sum_{(i,j)  \in S} \bv_{(i,j)} \bv_{(i,j)}^\top\right)$ is equal to the NSW objective. Our results not only recover the constant factor approximation to the NSW maximization problem shown in~\cite{anari2016nash}, but also allow us to give an $O(d)$-approximation when the allocation $(S_1, \ldots, S_d)$ is required to satisfy additional matroid constraints.  For example, the works~\cite{GourvesMT13,GourvesMT14,GourvesM19} considered allocations such that $\bigcup_{i = 1}^d S_i$ is a basis of a matroid $\M'$. We can model such a constraint by defining our constraint matroid $\M$ so that $S \subseteq [d] \times [m]$ is a basis of $\M$ if and only if $|\{i: (i,j) \in S\}| = 1$ for all $j \in [m]$ and $\{j: \exists i\text{ s.t. } (i,j) \in S\}$ is a basis of $\M'$. Our results then imply an $O(d)$-approximation for maximizing NSW subject to these, very general, matroid constraints.

\sasho{One other paper requires that each $S_i$ is a basis of a
  matroid $\M_i$. I don't see how to model this in our setup. Thoughts?}

%We are given a set of $m$ indivisible items, $n$ agents, and a utility for each item-agent pair $u_{i,j}, i \in [m], j \in [n]$. An allocation $\bx \in \{0,1\}^{n \times m}$ assigns each item to exactly one agent; for every $j$, $x_{ij}$ is $1$ for exactly one $i$ and $0$ otherwise. Value that a player $i$ receives is $u_i(\bx) = \sum_{j=1}^m u_{i,j}x_{i,j}$. The objective is to find an allocation $\bx$ which maximizes $\pr{\Pi_{i=1}^n u_i(\bx)}^{\frac{1}{n}}$. This is a special case of \DetMax{}. For each $i\in [n], j \in [m]$, we create a vector $\bv_{i,j}$ whose $i$-th entry is $\sqrt{u_{i,j}}$ and a partition matroid with partitions $\{\bv_{i,j} \mid i \in [n]\}_{j \in [m]}$. For an allocation $\bx \in \{0,1\}^n$, $\sum_{i=1}^n \sum_{j=1}^m x_{i,j} \bv_{i,j} \bv_{i,j}^\top$ is a diagonal matrix with $i$-th diagonal entry equal to the value that the player $i$ receives, i.e.$u_i(\bx)$.



==> app-finite.tex <==
%\subsection{Proof that \(\inf_{z\in\Z}\)  attains its minimum}

==> extra.tex <==
\section{Oblivious rounding scheme}\label{sec:no_pc_dist}

In this section, we show that none of the previous approaches for \DetMax\ yield an approximation factor independent of the size of the output solution $k$ even if the dimension of the vectors $d$ is $2$. Formally, we show that any relaxation and rounding schemes satisfying the following properties cannot achieve an approximation factor independent of $k$. 
\begin{itemize}
\item Let the relaxation be $\sup_{\bx \in \P(\M)} g(\bx)$ for some function $g$. Then, for any $\bx = \sum_{T \in \B} \lambda_T 1_T \in \P(\M)$, we have $g(\bx) \geq \max_{T \in \B} \det\pr{\lambda_T \sum_{i \in T} \bv_i \bv_i^\top}$.
\item Given $\bx \in \P(\M)$, the rounding scheme outputs a solution $T \in \B$ with probability dependent only on $\bx$ and $\M$ (and so independent of $\bv_i$'s). 
\end{itemize}

We construct an   instance as follow(s).
\paragraph{Matroid $\M$ and $\bx \in \P(\M)$:} Consider the graphic matroid with a graph $G$ on $n+2$ vertices $V = \{a_1,\dots,a_m\} \cup \{b,c\}$ and an edge set $E = \{a_ib,a_ic \mid i \in [m]\}$. All  spanning trees of $G$ are  bases of  matroid \(\M\). Consider a fractional spanning tree $\bx^\star$ such that $x_e^\star = \frac{m+1}{2m}$ for every edge $e \in E$. 

Let the rounding scheme picks a subset of edges with distribution $\mu :2^{E} \rightarrow \rR_+$. Since the rounding scheme outputs a basis of the matroid, it must be that $\mu(F) = 0$ if the graph $(V,F)$ has a cycle. Suppose we sample a subgraph as per distribution $\mu$. We let
\begin{center}
$B_i:=$ the event that both $a_ib$ and $a_ic$ are picked.
\end{center}
We prove some property about these events.
\begin{claim}For any $i \neq j$, $\Pr[B_i \cap B_j] = 0$. Hence, $\exists i \in [m]$ such that $\Pr[B_i] \leq \frac{1}{m}$.
\end{claim}
\begin{proof}
If both $B_i$ and $B_j$ occur, then our sampled subgraph contains edges $a_ib,a_ic,a_jb,a_jc$ which implies that there is a cycle in the subgraph. However, as per the definition $\mu(F) = 0$ if the sampled subgraph $(V,F)$ has a cycle. Hence, $\Pr[B_i \cap B_j] =0$. So, $\sum_{i=1}^m \Pr[B_i] =\Pr[\cup_{i=1}^m B_i] 
 \leq 1$, and there exists  $i \in [m]$ such that $\Pr[B_i] \leq \frac{1}{m}$. 
\end{proof}

We continue constructing the instance with descriptions of input vectors.
\paragraph{Vector Set:} Consider the vector set as follows: $\bv_{a_ib} = \left[\begin{array}{c} 2\\ 0\end{array}\right], \bv_{a_ic} = \left[\begin{array}{c} 0 \\ 2 \end{array}\right]$, and for $j \neq i$, $\bv_{a_jb} = \bv_{a_jc} = \left[ \begin{array}{c} 0 \\ 0 \end{array} \right]$. Since the rounding scheme is oblivious to the set of vectors, we can make such a selection.

By the assumption on our relaxation, we have that $g(\bx^\star) \geq \det\pr{\frac{m+1}{2m}\bv_{a_ib} \bv_{a_ib}^\top + \frac{m+1}{2m}\bv_{a_ic}\bv_{a_ic}^\top} = \frac{(m+1)^2}{m^2} >1$. The rounding scheme with distribution $\mu$ outputs a solution with non-zero value only if both $a_i u$ and $a_iv$ are picked. Hence, the expected objective value of the solution returned is 
\[\Pr[B_i] \det\pr{\bv_{a_ib}\bv_{a_ib}^\top + \bv_{a_ic}\bv_{a_ic}^\top} \leq \frac{4}{m}\] 
and the approximation factor achieved is larger than $\frac{1}{\frac{4}{m}} = \frac{m}{4}$. As $m \rightarrow \infty$, the approximation factor tends to infinity even for $d=2$. 

To construct a similar instance for $d>2$, we  add vectors $\bv_i = \left[\begin{array}{c} 0^{i-1}\\ 1 \\ 0^{d-i}\end{array}\right]$ for  each $i \in \{3,\dots,d\}$ and include them in  the bases of the matroid.


%
%
% that for any concave relaxation and any rounding scheme which does not consider the structure of the vectors yields an algorithm with approximation factor dependent on $k$ even for $d=2$.
%
%\begin{definition}
%A rounding scheme is oblivious if the probability of outputting a solution $T \subseteq V$ depends only on the matroid $\M = (\V,\I)$ and the fractional solution $\bx\in \P(\M)$ and is independent of the vector set $v_1,\dots,v_n$.
%\end{definition}
%
%\begin{definition}
%A relaxation $\sup_{\bx \in \P(\M)} g(\bx)$ is \crel if for any matroid $\M$, vector set $v_1,\dots,v_n$ and $\bx \in \P(\M)$, $g(\bx) \geq \max_{T \in \B}\det\pr{\lambda_T\sum_{i \in T} \bv_i \bv_i^\top}$ where $\bx = \sum_{T \in \B} \lambda_T 1_T$.
%\end{definition}
%
%\begin{theorem}
%For any function $f: \nN \rightarrow \nN$, any \crel relaxation , and any oblivious rounding scheme, there exists an instance with matroid $\M = (V,\I)$, vectors set $v_1,\dots,v_n \in \rR^2$ and a fractional solution $\bx^\star \in \P(\M)$ with value of the concave relaxation at least $1$ such that expected objective value of the solution returned is less than $1/f(d)$.
%\end{theorem}
%\begin{proof}
%Let the relaxation be
%\[ \sup_{\bx \in \P(\M)} g(\bx)\]
%Consider the graphic matroid with a graph $G$ on $n+2$ vertices $V = \{a_1,\dots,a_m\} \cup \{b,c\}$ and edge set $E = \{a_ib,a_ic \mid i \in [m]\}$. All the spanning trees of $G$ are the bases of the matroid. Consider a fractional spanning tree $\bx^\star$ such that $x_e^\star = \frac{m+1}{2m}$ for every edge $e \in E$. Let the rounding scheme picks a subset of edges with distribution $\mu :2^{E} \rightarrow \rR_+$ such that $\mu(F) = 0$ if the graph $(V,F)$ has a cycle. Suppose, we sample a subgraph as per distribution $\mu$. For $i \in [m]$, let
%\begin{center}
%$B_i:=$ event that both $a_ib$ and $a_ic$ are picked.
%\end{center}
%\begin{claim}For any $i \neq j$, $Pr[B_i \cap B_j] = 0$. Hence, $\sum_{i=1}^m Pr[B_i] \leq 1$.
%\end{claim}
%\begin{proof}
%If both $B_i$ and $B_j$ occur, then our sampled subgraph contains edges $a_ib,a_ic,a_jb,a_jc$ which implies that there is a cycle in the subgraph. However, as per the definition $\mu(F) = 0$ if the sampled subgraph $(V,F)$ has a cycle. Hence, $Pr[B_i \cap B_j] =0$.
%\end{proof}
%This implies that there exists an $i \in [m]$ such that $Pr[B_i] \leq \frac{1}{m}$. Consider a vector set as follows: $v_{a_ib} = \left[\begin{array}{c} 2\\ 0\end{array}\right], v_{a_ic} = \left[\begin{array}{c} 0 \\ 2 \end{array}\right]$ and for $j \neq i$, $v_{a_jb} = v_{a_jc} = \left[ \begin{array}{c} 0 \\ 0 \end{array} \right]$. Since the rounding scheme is oblivious to the set of vectors, we can make such a selection.
%
%Since the relaxation is \crel, $g(\bx^\star) \geq \det\pr{\frac{m+1}{2m}v_{a_ib} v_{a_ib}^\top + \frac{m+1}{2m}v_{a_ic}v_{a_ic}^\top} = \frac{(m+1)^2}{m^2} >1$. Rounding scheme with distribution $\mu$ outputs a solution with non-zero value only if both $a_i u$ and $a_iv$ are picked. Hence, expected objective value of the solution returned is $Pr[B_i] \det\pr{v_{a_ib}v_{a_ib}^\top + v_{a_ic}v_{a_ic}^\top} \leq \frac{4}{m}$. So, for any function $f:\nN \rightarrow \nN$, we can select a large enough $m$ such that $\frac{4}{m} <\frac{1}{f(2)}$.
%\end{proof}
%
%To construct similar instance for $d>2$, we can add vectors $\bv_i = \left[\begin{array}{c} 0^{i-1}\\ 1 \\ 0^{d-i}\end{array}\right]$ for $i \in \{3,\dots,d\}$ and include them in all the bases of the matroid.
%
%\begin{remark}
%All the approaches considered before in the context of real stable polynomials or log-concave polynomials make use of oblivious rounding schemes and \crel relaxations. Hence, those approaches can not yield an approximation factor independent of $k$.
%\end{remark} 





==> future.tex <==
\section{Conclusion and Future work}
In this paper, we showed that none of the previous works on \DetMax\ for general matroid can yield estimation and approximation factors independent of $k$, the size of the output set. We showed an $\pr{O(d)}^d$-estimation algorithm by first showing the existence of an optimal solution to the convex program with at most $O(d^2)$ strictly fractional variables and rounding such a fractional solution. To improve this estimation factor, we may try answering the following question:

\begin{quest}
Let $\M=([n],\I)$ be a matroid with bases $\B$ and let $\bx^\star \in \P(\M)$ be a point in the matroid bases polytope with at most $O(d^2)$ strictly fractional variables, i.e. $|\{i\in [n] : 0 < x_i^\star < 1\}|  = O(d^2)$. For any $d$, does there always exist a distribution $\mu:\B \rightarrow \rR_+$ such that for any independent set $S$ of size $d$,
\[ \Pr_{T \sim \mu}[S \subseteq T] \geq e^{-O(d)} \Pi_{i \in S} x_i^\star ?\]
\end{quest}

A positive resolution to this question would improve the estimation factor for \DetMax{} problem from $\pr{O(d)}^d$ to $\pr{O(1)}^d$. 


==> overview.tex <==
\section{Paper overview}
Let $v_1,\dots,v_n \in \rR^d$ be $d$-dimensional vectors and $\M = ([n],\I)$ be a matroid with bases set $\B \subset \I$ Our goal is to find $T \in \B$ such that $det\pr{\sum_{i\in T} v_i v_i^\top}$ is maximized. This problem is NP-hard in the most restrictive setting such as when $\M$ is a uniform matroid. So, we focus on approximation algorithms for the problem. In this paper, we design approximation algorithms using concave relaxations. That is, we solve the following program:
\begin{equation}\label{eq:generic_rel}
 \sup_{\bx \in P(M)} f(\bx)
\end{equation}
where $P(M)$ is the matroid bases polytope and $f(\bx)$ is a function such that for any integral point $\bx \in P(M)$, $f(\bx) \geq det\pr{\sum_{i=1}^n x_i v_i v_i^\top}$. We then design a rounding scheme which given a fractional point $\bx^* \in P(M)$, find an integral point $\bx' \in P(M)$ such that $det\pr{\sum_{i=1}^n x_i' v_i v_i^\top} \geq \alpha f(\bx^*)$.  This yields an $\alpha$-approximation algorithm if the rounding scheme is efficient and we can solve \eqref{eq:generic_rel} efficiently. A natural choice for $f(\bx)$ is $det\pr{\sum_{i=1}^n x_i v_i v_i^\top}$. Unfortunately, this gives a relaxation with unbounded integrality gap. Consider a partition matroid with partitions $P_1 = \{1\}, P_2 = \{2,3\}$ and vectors $v_1 = \begin{bmatrix} 0 \\ 0 \end{bmatrix}, v_2 = \begin{bmatrix} 1\\0\end{bmatrix}, v_3 = \begin{bmatrix} 0 \\ 1\end{bmatrix}$. Any integral solution would pick $v_1$ and either $v_2$ or $v_3$. Value of both of these solutions is zero. However, a fractional solution $x_1 = 1, x_2 = x_3 = \frac{1}{2}$ is in the matroid bases polytope and has non-zero value. This suggests that we require a stronger relaxation. Nikolov and Singh~\cite{NikolovS16} proposed one such relaxation based on the following observations:
\begin{itemize}
\item Cauchy-Binet formula shows that $det\pr{\sum_{i=1}^n x_i v_i v_i^\top} = \sum_{S \in {[n] \choose d}} x^S det\pr{\sum_{i \in S} v_i v_i^\top}$ where $x^S = \Pi_{i \in S} x_i$.
\item For any basis $T$ of the matroid, all subsets $S \subseteq T$ are independent. Hence, for any integral solution $\bx$, $x^S$ is non-zero only if $S$ is an independent set.
\end{itemize}
Based on these observations Nikolov \etal~\cite{NikolovS16} wrote the following relaxation:
\begin{equation}\label{eq:nikolovs_rel}
 \sup_{\bx \in P(M)} \inf_{\by \in \rR_+^n: \forall S \in \I_d, y^S \geq 1} \sum_{S \in {[n] \choose d}} x^S y^S det\pr{\sum_{i \in S} v_i v_i^\top} = det\pr{\sum_{i=1}^n x_i y_i v_i v_i^\top}
\end{equation}

\[ \sup_{\bx \in P(M)} \inf_{\by: \forall S \in \I_d, y^S \geq 1} x^S y^S det\pr{\sum_{i \in S} v_i v_i^\top}\]
where $\I_d$ is the set of independent sets of size $d$. This was inspired by a similar relaxation for permanent by Gurvits~\cite{Gurvits08}. Next, to design a rounding scheme we need the notion of a positively correlated distribution.

\begin{definition}
For a matroid $\M$ and $x \in P(\M)$, we say that a distribution $\mu \in [0,1]^\B$ is $(\alpha,d)$-positively correlated if for any independent set $S \in \I_d$,
\[ P_{T \sim \mu} [S \subset T] \geq \alpha\cdot x^S.\]
\end{definition}
\vivek{@everyone: Suggest a better terminology.}

If there exists an $(\alpha,d)$ positively correlated distribution, we can round the fractional solution of \eqref{eq:nikolovs_rel} to get an integral solution with value
\begin{align*}
E_{T \sim \mu} \left[ det\pr{\sum_{i \in T} v_i v_i^\top}\right] &= E_{T \sim \mu} \left[ \sum_{S \in {T \choose d}} det\pr{\sum_{i \in S} v_i v_i^\top}\right]\\
& = \sum_{S \in \I_d} Pr_{T \sim \mu} [S \subseteq T] det\pr{\sum_{i \in S} v_i v_i^\top}\\
& \geq \alpha \sum_{S \in \I_d} x^S det\pr{\sum_{i \in S} v_i v_i^\top}
\end{align*}
Nikolov and Singh~\cite{NikolovS16} showed the existence of $(1,d)$-positively correlated distribution for partition matroid of rank $d$. Using the theory of real stability, they further showed that for any $\bx \in \rR_+^n$ and partition matroid of any rank,
\begin{equation}\label{eq:nikolovs_main_result}
\sum_{S \in \I_d} x^S det\pr{\sum_{i \in S} v_i v_i^\top} \geq e^{-d} \inf_{y \in \rR_+^n: \forall S \in \I_d, y^S \geq 1} det\pr{\sum_{i =1}^n x_i y_i v_i v_i^\top}
\end{equation}
Again, this was an extension of the work by Gurvits~\cite{Gurvits08} on real stable polynomials. This result combined with $(1,d)$-positively correlated distribution for partition matroid of rank $d$ gives an $e^{-d}$-approximation algorithm for \Ddesign with partition matroid of rank $d$. In this paper, we show the existence of $(e^{-d},d)$-positively correlated distributions for partition matroid of any rank. This yields the following result:
\begin{theorem}
There exists an $e^{-2d}$ approximation algorithm for partition matroid of arbitrary rank.
\end{theorem}

Generalizing this result for arbitrary matroids hasn't been easy. There are two main issues. First issue is that unlike partition matroid, the generating polynomial for arbitrary matroid is not real stable and hence \eqref{eq:nikolovs_main_result} is not valid for arbitrary matroid. This is not hard to resolve. There have been a series of work generalizing the result for real stable polynomials to log-concave polynomials~\cite{AnariGV18,AnariLGV19}. From this work, we can relate the output of the rounding scheme to a different relaxation considered in \cite{AnariGV18} for optimization using the theory of log-concave polynomials. Anari \etal~\cite{AnariGV18} proved that for any matroid $\M$ and $\bx \in P(\M)$,
\begin{equation}\label{eq:cost_anarig_rel}
 \sum_{S \in \I_d} x^S det\pr{\sum_{i \in S} v_i v_i^\top}  \geq e^{-2d} \sup_{\alpha \in P(\M)} \inf_{y,z \geq 0} \frac{det\pr{\sum_{i=1}^nx_i y_i v_i v_i^\top}\pr{\sum_{S \in \I_d} z^S} }{\pr{\frac{\by\bz}{\alpha}}^\alpha}
\end{equation}
In this paper, we show that \eqref{eq:nikolovs_rel} is stronger than this relaxation. That is, for any matroid $\M$ and $\bx \in P(\M)$,
\begin{equation}\label{eq:anari_nikolov_rel}
\sup_{\alpha \in P(\M)} \inf_{y,z \geq 0} \frac{det\pr{\sum_{i=1}^nx_i y_i v_i v_i^\top}\pr{\sum_{S \in \I_d} z^S} }{\pr{\frac{\by\bz}{\alpha}}^\alpha} \geq
\inf_{\by \in \rR_+^n: \forall S \in \I_d, y^S \geq 1}det\pr{\sum_{i=1}^n x_i y_i v_i v_i^\top}
\end{equation}
Second issue in generalizing the result from partition matroid to arbitrary matroid is the fact that there does not exists a $(\alpha,d)$ positively correlated distribution where $\alpha$ is a function of $d$. More formally,
\begin{theorem}
For any function $g: \nN \rightarrow \nN$, there exists a matroid $\M$ and $\bx \in P(\M)$ which does not admit a $(g(d),d)$-positively correlated distribution.
\end{theorem}
This turned out to be significantly harder issue to resolve. We resolve it in two steps. First is a new algorithm showing the exists of a $(g(d),d)$-positively correlated distribution if the solution $\bx$ is sparse. Second, we show the existence of a sparse optimal solution.

\vivek{We need some text to emphasize that showing sparsity for our program is not easy.}

\begin{definition}
A solution $\bx \in P(\M)$ is said to be $\beta$-sparse if the number of fractional values is at most $\beta$. That is,
\[ |\{i \in [n]\mid 0 < x_i < 1\}| \leq \beta\]
\end{definition}

\begin{theorem}\label{thm:sparse_distribution}
For any matroid $\M$ and $2(d^2+d)$-sparse solution $\bx \in P(\M)$, there exists a $\left(e^{-1.5} (2e^3 d)^{-d},d\right)$-positively correlated distribution.
\end{theorem}

Next, to show sparsity of optimal solution we start by proving the optimality condition for $\inf_{y \in \rR_+^n:\forall S \in \I_d, y^S \geq 1} det\pr{\sum_{i=1}^n x_i y_i v_i v_i^\top}$.

\begin{theorem}Let $Y = \{ y \in \rR_+^n \mid \forall S \in \I_d, y^S \geq 1\}$.  For $x^* \in P(\M)$ and $y^* \in Y$,  let $X = \sum_{i=1}^n x_i^* y_i^* v_i v_i^\top$ and $w_i = x_i^* y_i^* v_i^\top X^{-1} v_i$ for $i \in [n]$. Let $\B^* = \{S \in \I_d \mid (y^*)^S = 1\}$ and $\M^*$ be the matroid with basis set $\B^*$. Then,
\begin{center}
$\by^* \in \argmin_{y  \in Y}  det\pr{\sum_{i=1}^n x_i^* y_i v_i v_i^\top}$ iff $\bw \in P(\M^*)$.
\end{center}
\end{theorem}

Now, suppose $(\bx^*, \by^*)$ is an optimal solution to  the relaxation \eqref{eq:nikolovs_rel} and $\M^*$ be as defined in the theorem above. If we can find a solution $\bx' \in P(\M)$ such that $\bw' \in P(\M^*)$ where $w_j' = x_j' y_j^* v_j^\top \pr{\sum_{i=1}^n x_i' y_i^* v_i v_i^\top}^{-1}  v_j$, then $\by^* \in \argmin_{y  \in Y}  det\pr{\sum_{i=1}^n x_i' y_i v_i v_i^\top}$. Moreover, if $\sum_{i=1}^n x_i' y_i^* v_i v_i^\top = \sum_{i=1}^n x_i^* y_i^* v_i v_i^\top$, then $(x',y^*)$ is an optimal solution to the relaxation \eqref{eq:nikolovs_rel} as well.

\begin{figure}
\centering
\begin{boxedminipage}{0.5\textwidth}
\begin{align*}
&\bx \in P(\M)\\
& \bw \in P(\M^*) \text{ where } w_j = x_jy_j^* v_j^\top \pr{\sum_{i=1}^n x_i^* y_i^* v_i v_i^\top}^{-1} v_j\\
&\sum_{i=1}^n x_i y_i^* v_i v_i^\top = \sum_{i=1}^n x_i^* y_i^* v_i v_i^\top
\end{align*}
\end{boxedminipage}
\caption{}
\label{fig:sparsify_lp}
\end{figure}

\begin{theorem}
Let $(\bx^*,\by^*)$ be an optimal solution to \eqref{eq:nikolovs_rel}. Let $\M^*$ be the matroid with basis set $\{ S \in \I_d \mid (y^*)^S = 1\}$. Let $\bx'$ be a solution to LP~\ref{fig:sparsify_lp}. Then, $(\bx',\by^*)$ is an optimal solution to \eqref{eq:nikolovs_rel}.
\end{theorem}

\begin{theorem}
Any extreme point of the polytope defined by LP~\ref{fig:sparsify_lp} has at most $2(d^2+d)$ fractional values.
\end{theorem}

From these two theorems, we can conclude that there exists a sparse optimum solution to \eqref{eq:nikolovs_rel}.

\begin{corollary}
There exists an optimal solution $(\bx',\by^*)$ to \eqref{eq:nikolovs_rel} such that
\[|\{i \in [n]\mid 0<x_i' < 1\}| \leq 2(d^2 + d).\]
\end{corollary}

Combining this corollary with Theorem~\ref{thm:sparse_distribution}, \eqref{eq:cost_anarig_rel}, and \eqref{eq:anari_nikolov_rel}, we get the main result of this paper:

\begin{theorem}
There exists a $e^{-1.5}(2e^5d)^{-d}$-approximation algorithm for \Ddesign with arbitrary matroid.
\end{theorem}


\begin{remark}
Results mentioned above by Gurvits~\cite{Gurvits08}, Nikolov \etal~\cite{NikolovS14}, and Anari\etal~\cite{AnariGV18} are not restricted to the \Ddesign problem but apply more generally to the real stable and log-concave polynomials.
\end{remark}

\para{Inf vs min:}


\para{Solving the relaxation:}


==> related.tex <==
\subsection{Related Work}

\paragraph{Uniform Matroid:} \DetMax{} is NP-hard even for uniform matroid ~\cite{Welch82}. Koutis~\cite{Koutis06} showed that there exists a constant $c>0$ such that it is NP-hard to approximate better than a factor of $(1+c)^d$~\cite{Koutis06}.  Let $k$ be the rank of the uniform matroid. Bouhtou \etal ~\cite{BouhtouGS10} gave a $\pr{\frac{n}{k}}^d$-approximation algorithm based on rounding the solution of a natural concave relaxation. Nikolov~\cite{Nikolov15} improved the result to a $e^{k}$-approximation when $k \leq d$. Wang \etal~\cite{WangYS16} improved the approximation ratio of $(1+\epsilon)^d$ when $k \geq \frac{d^2}{\epsilon}$. Allen-Zhu \etal~\cite{Allen-Zhu2017} improved the bound on $k$ to give $(1+\epsilon)^d$-approximation when $k = \Omega\pr{\frac{d}{\epsilon^2}}$. This was improved by Singh \etal~\cite{SinghX18} who gave a $(1+\epsilon)^d$-approximation when $k = \Omega\pr{\frac{d}{\epsilon} + \frac{1}{\epsilon^2} \log \frac{1}{\epsilon}}$. Recently, this was improved by Madan\etal~\cite{MadanSTU19} who gave a $(1+\epsilon)^d$-approximation when $k \geq d + \frac{d}{\epsilon}$.

\paragraph{General Matroid:} Nikolov and Singh~\cite{NikolovS16} gave a $e^d$-approximation for \DetMax{} with partition matroid of rank $d$. Let $k$ be the rank of a general matroid. Anari and Gharan~\cite{anari2017generalization} gave a $e^{2k}$-approximation when the generating polynomial for the matroid is real-stable. This corresponds to the Strongly Rayleigh matroids which includes both uniform and partition matroids. This was generalized by Anari, Gharan, and Vinzant~\cite{AnariGV18} who gave a $e^{2k}$-approximation for any matroid. While the result in~\cite{AnariGV18} is not stated for $k>d$, it can be easily deduced from the analysis. Algorithms in~\cite{NikolovS16,anari2017generalization,AnariGV18} are estimation algorithms as they estimate the optimum value up to a certain approximation factor, but do not yield a solution in polynomial time. Straszak and Vishnoi~\cite{straszak2017real} gave a polynomial time algorithm without output a $O(\sqrt{k} e^k)$-approximate solution for partition matroid.


==> relaxation.tex <==
\section{Relaxation}
\vivek{This section can be deleted as the next section discuss these in more details.}
Let the set of vectors be $V=\{v_1,\dots,v_n\}$.  For a matroid \(\M=([n],\I)\), we denote
\(\I_s(\M)=\set{S\in\I:|S|=s}\), the set of all independent sets of
size \(s\). We denote by \(\P(\M)\) the matroid base polytope of
\(\M\). For any vector \(z\in\R^{[n]}\) of real numbers indexed by \([n]\)
and a subset \(S\subseteq [n]\), we denote \(z(S)=\sum_{i\in S} z_i\). Let $\Z = \{ z \in \rR^{[n]} : \forall S \in \I_d(M), z(S) \geq 0\}$. We now introduce an optimization problem
\begin{equation} \label{eq:D-relax}
\max_{\bx\in\P(\M)}  \inf_{z\in\Z} g(x,z):= \log\det\pr{\sum_{i \in [n]} x_ie^{z_i} v_i v_i^\top}
\end{equation}
\vivek{It should be sup instead of max, correct? Not obvious as to why sup is equal to max.}

We call the optimization problem \eqref{eq:D-relax} \CPD{($\M,V$)}. We denote
its optimum value by \CP{($\M,V$)} and optimal solution (when one exists) by
\((x^\star,z^\star)\).

\begin{theorem}\label{thm:relax}
\eqref{eq:D-relax} is a relaxation for \Ddesign (\vivek{not correct}). That is,
\[\DOPT{(\M,V)} \leq \exp(\CP{(\M,V)})\]
for any set of vectors $V = \{v_1,\dots,v_n\}$ and matroid $\M=([n],\I)\}$.
\end{theorem}

The next theorem shows that \CPD{} can be solved approximately to any
degree of accuracy.

\begin{theorem} \label{thm:solvability}
There is an algorithm that given an instance of the \DOPT{} problem and $\epsilon>0$ either shows that the optimal value is $0$ or returns a solution to $(\tilde{x},\tilde{z})$ such that
\begin{enumerate}
\item $f(\tilde{x})\geq f(x^\star) -\epsilon$.
\item $g(\tilde{x}, \tilde{z})\leq \inf_{{z\in\Z}} g(\tilde{x}, z)+\epsilon.$
\item \ms{We need some for approximate KKT.} \sasho{For now we are not
    doing approximate KKT, are we?}
\end{enumerate}
The algorithm runs in polynomial time in the size of the input and \(\log\pr{\frac 1\eps}\).
\end{theorem}

For $\bx \in \P(\M)$, let $$f(\bx):=
\inf_{\bz\in\Z} g(\bx,\bz).$$
Let $\bx^* \in \P(\M)$ be the optimum solution to \CPD. As discussed above, our rounding algorithm yields a positively correlated distribution if $\bx^*$ is sparse which may not always be the case. In order to convert the $\bx^*$ into a sparse optimum solution $\bx'$, we need the existence of finite $\bz^*$ optimizing $f(\bx^*)$; $g(\bx^*,\bz^*) = f(\bx^*)$. However, for some of the \Ddesign instances and optimum $\bx^*$, there may not exists any finite optimum $\bz^*$.  This issue can be resolved using the following lemma:

\begin{lemma} \label{lem:finite_z}
  Let \(\hat \bx\in\P(\M)\) be such that $\max_{i \in [n]}, \hat x_i < 1$,
  \(f(\hat \bx)=\inf_{\bz\in\Z} g(\hat \bx,\bz)\) is finite, and suppose that
  the vectors $\{v_i: i\in [n]\}$ are in general position. Then,
  \(g(\hat \bx,\bz)\) attains its infimum over \(\bz\in\Z\) at some
  \(z^*\in\Z\). Here, vectors $\{v_i: i \in [n]\}$ in general position means that all subset of vectors of size $d$ are linearly independent.
\end{lemma}

Next, given a \Ddesign instance with vectors $V=\{v_1,\dots,v_n\}$ and matroid $\M = ([n],\I)$, we can create a \Ddesign instance with vectors $V' = \{v_1',\dots,v_m'\}$ and matroid $\M' = ([m],\I')$ such that both the optimum and the relaxation optimum are roughly same for both instances. Additionally, vectors $V'$ are in general position and there exists an optimum solution $\bx^*\in \P(\M')$ to the relaxation with $V', \M'$ satisfying $\max_{i \in [m]} x_i < 1$.

\begin{lemma}\label{lem:new_instance}
For any $\epsilon > 0$, given a matroid $\M  = ([n],\I)$ an vector set $V= \{v_1,\dots,v_n\}$, we can construct $\M' = ([m], \I')$ and $V' = \{v_1',\dots,v_m'\}$ in time $poly\pr{n,d,\frac{1}{\epsilon}}$ such that
\begin{itemize}
\item $|\CP(\M,V) - \CP(\M',V')| < \epsilon$ and $\frac{\DOPT{(\M,V)}}{\DOPT(\M',V')} \in [1-\epsilon, 1+\epsilon]$.
\item Vectors $\{ v_1',\dots,v_m'\}$ are in general position.
\item There exists $\hat \bx$ with $\max_{i\in [m]} \hat x_i < 1$ which is approximately optimal for \CPD with matroid $\M'$ and vector set $V'$. That is,  $\inf_{z\in\Z'} g(\hat x,z) \geq \sup_{x \in \P(\M')} \inf_{z \in \Z'} g(\bx,\bz)$ where $\Z' = \{ \bz \in \rR^{[m]} : \forall S \in \I_d(\M'), z(S) \geq 0\}$.
\end{itemize}
\end{lemma}

\vivek{If we require general position for solvability, we can delete Theorem~\ref{thm:solvability} and another part to Lemma~\ref{lem:new_instance} stating that the relaxation can be solved for $(\M',V')$.}

Due to Lemma~\ref{lem:finite_z} an Lemma~\ref{lem:new_instance}, we can assume (at the loss of a $1+\epsilon$ factor) that for our instance $(\M,V)$, there exists an optimum solution $\bx^*$ such that $f(\bx^*) = \inf_{\bz \in \Z} g(x^*, \bz)$ is achieved at finite $\bz^*$. Proof of Theorem~\ref{thm:relax}, Theorem~\ref{thm:solvability}, Lemma~\ref{lem:finite_z}, an Lemma~\ref{lem:new_instance} is deferred to the Appendix.

\vivek{Replace $P$ with $\P$ everywhere. Check for consistency in notation $\P(\M)$ and $\P_{\M}$. } 

